TinyFlow: Breaking the Warping Bottleneck for Edge Optical Flow

High-performance optical flow networks are difficult to deploy on resource-constrained edge accelerators because their iterative refinement warps features by the current flow, which relies on flow-dependent resampling and data-dependent memory access. We present TinyFlow, a 1.26M-parameter warp-free optical flow network that preserves iterative coarse-to-fine refinement by replacing the warp with a fixed-window correlation over constant offsets, so the whole network compiles as a single static INT8 graph. Quantization-aware fine-tuning, warp-teacher distillation, and model souping reduce the Float32-to-INT8 penalty to below 0.2 end-point error (EPE) on MPI-Sintel. TinyFlow outperforms EdgeFlowNet and NanoFlowNet on Sintel Clean, Sintel Final, and FlyingChairs in both Float32 and INT8, while using 54% fewer parameters than EdgeFlowNet, and our INT8 model achieves 6.29/7.13 EPE on Sintel Clean/Final. In flow-only monocular visual odometry on TartanAir and UZH-FPV, the same INT8 model yields the lowest trajectory error on seven of eleven sequences.

==> sections/4_0_quantizedmodel_redesign.tex <==
\section{Quantization-Oriented Model Redesign\\
\textcolor{red}{check if this part is needed later}}
\label{sec:quantization_redesign}

The original TinyFlow model was designed to be warp-free and exportable, but several components were still unfriendly to INT8 deployment on Hailo. 

In particular, the original backbone used depthwise separable convolution blocks without batch normalization, and the residual blocks directly added the residual branch to the skip connection:
\begin{equation}
\mathbf{x}_{\mathrm{out}} = \mathbf{x} + \mathcal{F}(\mathbf{x}).
\end{equation}
Although ReLU6 was used inside the convolution blocks, the residual accumulation itself was not bounded. This caused large activation ranges and frequent output-bit reduction warnings during Hailo quantization.

To improve quantization stability, we redesigned the backbone using batch-normalized depthwise separable blocks. Each depthwise and pointwise convolution is followed by batch normalization and ReLU6:
% \begin{equation}
% \begin{aligned}
% \mathrm{DWConvQ}(\mathbf{x})
% =
% \mathrm{ReLU6}\Big(
% \mathrm{BN}\big(
% \mathrm{PWConv}(
% \mathrm{ReLU6}(
% \mathrm{BN}(
% \mathrm{DWConv}(\mathbf{x})
% )))
% \big)
% \Big).
% \end{aligned}
% \end{equation}


\begin{equation}
\begin{aligned}
\operatorname{DWConvQ}(\mathbf{x})
&= \operatorname{ReLU6}\!\Big(
   \operatorname{BN}\big(
   \operatorname{PWConv}(\mathbf{z})
   \big)
   \Big), \\
\mathbf{z}
&= \operatorname{ReLU6}\!\Big(
   \operatorname{BN}\big(
   \operatorname{DWConv}(\mathbf{x})
   \big)
   \Big).
\end{aligned}
\end{equation}

We also added batch normalization to the backbone stem. The residual block was changed to apply a bounded activation after the residual addition:
\begin{equation}
\mathbf{x}_{\mathrm{out}}
=
\mathrm{ReLU6}\left(\mathbf{x} + \mathcal{F}(\mathbf{x})\right).
\end{equation}
This prevents the residual outputs from growing without bound and makes the intermediate feature distributions more suitable for INT8 quantization.

% The original model also used channel-wise L2 normalization before correlation:
% % \begin{equation}
% % \hat{\mathbf{f}}
% % =
% % \frac{\mathbf{f}}
% % {\sqrt{\sum_{c} \mathbf{f}*{c}^{2} + \epsilon}} .
% % \end{equation}
% \begin{equation}
% \hat{\mathbf{f}}
% =
% \frac{\mathbf{f}}
% {\sqrt{\sum_{c} \mathbf{f}_{c}^{2} + \epsilon}} .
% \end{equation}


% Although this normalization is effective in floating-point training, it introduces dynamic square-root and division operations that are less hardware-friendly. We therefore replaced it with a learnable feature projector:

% \begin{equation}
% \hat{\mathbf{f}}
% =
% \frac{1}{\sqrt{C}}
% \mathrm{BN}\left(
% \mathrm{Conv}_{1 \times 1}(\mathbf{f})
% \right),
% \end{equation}




% where $C$ is the number of channels. The $1 \times 1$ convolution is initialized as an identity mapping. This module approximates feature normalization using only convolution, batch normalization, and a fixed scaling factor, avoiding dynamic normalization operations.





We further redesigned the flow prediction heads and update blocks. In the original model, the flow heads directly regressed an unbounded two-channel flow output using a final convolution. This caused poor quantization behavior because the signed regression output could contain outliers.

In the quantization-oriented model, batch normalization is inserted after each hidden convolution in the coarse flow head and both refinement update blocks. Specifically, \texttt{FlowHead16}, \texttt{UpdateBlock8}, and \texttt{UpdateBlock4} all use the structure:
\begin{equation}
\mathrm{Conv}
\rightarrow
\mathrm{BN}
\rightarrow
\mathrm{ReLU6}
\rightarrow
\mathrm{Conv}
\rightarrow
\mathrm{BN}
\rightarrow
\mathrm{ReLU6}
\rightarrow
\mathrm{Conv}_{2}.
\end{equation}
Here, the final \(\mathrm{Conv}_{2}\) produces the two-channel horizontal and vertical flow output.

% The final regression output is then bounded using a scaled hyperbolic tangent:
% \begin{equation}
% \Delta \mathbf{u}
% =
% s \cdot \tanh\left(
% \frac{\mathcal{H}(\mathbf{x})}{s}
% \right),
% \end{equation}
% where \(\mathcal{H}\) is the convolutional prediction head and \(s\) controls the maximum output range. In our final model, the initial \(1/16\)-resolution flow head uses \(s=4\), the \(1/8\)-resolution update block uses \(s=2\), and the \(1/4\)-resolution update block uses \(s=1\). Therefore, the settings are:
% \begin{equation}
% s_{16}=4,\qquad s_{8}=2,\qquad s_{4}=1 .
% \end{equation}
% This design keeps the flow regression outputs numerically stable while still allowing multi-stage flow refinement.









% Finally, we changed the training loss to provide stronger supervision to the intermediate flow predictions. The original loss placed relatively small weights on the coarse predictions:
% % \begin{align}
% % \mathcal{L}*{\mathrm{old}}
% % =
% % &; 0.05,\mathcal{L}*{16}
% % + 0.2,\mathcal{L}*{8}
% % + w*{\mathrm{occ}},\mathcal{L}*{4}
% % + 0.05,\mathcal{L}*{\mathrm{ds8}} \notag \
% % &; + 0.1,\mathcal{L}*{\mathrm{ds4}}
% % + w*{\mathrm{sm}},\mathcal{L}*{\mathrm{smooth}} .
% % \end{align}


% \begin{equation}
% \begin{aligned}
% \mathcal{L}^{\mathrm{old}}
% =&\ 0.05\,\mathcal{L}_{16}
%  + 0.2\,\mathcal{L}_{8}
%  + w_{\mathrm{occ}}\,\mathcal{L}_{4} \\
% &+ 0.05\,\mathcal{L}_{\mathrm{ds8}}
%  + 0.1\,\mathcal{L}_{\mathrm{ds4}}
%  + w_{\mathrm{sm}}\,\mathcal{L}_{\mathrm{smooth}} .
% \end{aligned}
% \end{equation}




% In the final model, we increase the weights of the $1/16$ and $1/8$ flow losses:
% % \begin{align}
% % \mathcal{L}*{\mathrm{new}}
% % =
% % &; 0.4,\mathcal{L}*{16}
% % + 0.8,\mathcal{L}*{8}
% % + w_{\mathrm{occ}},\mathcal{L}*{4}
% % + 0.05,\mathcal{L}*{\mathrm{ds8}} \notag \
% % &; + 0.1,\mathcal{L}*{\mathrm{ds4}}
% % + w*{\mathrm{sm}},\mathcal{L}_{\mathrm{smooth}} .
% % \end{align}


% \begin{equation}
% \begin{aligned}
% \mathcal{L}^{\mathrm{new}}
% =&\ 0.4\,\mathcal{L}_{16}
%  + 0.8\,\mathcal{L}_{8}
%  + w_{\mathrm{occ}}\,\mathcal{L}_{4} \\
% &+ 0.05\,\mathcal{L}_{\mathrm{ds8}}
%  + 0.1\,\mathcal{L}_{\mathrm{ds4}}
%  + w_{\mathrm{sm}}\,\mathcal{L}_{\mathrm{smooth}} .
% \end{aligned}
% \end{equation}

% This encourages the coarse stages to produce meaningful flow estimates instead of relying only on the final $1/4$ refinement stage. As a result, the intermediate representations become more stable and easier to quantize.

% In practice, this stronger intermediate supervision was important for quantization because it encouraged the \(1/16\) and \(1/8\) stages to produce stable and meaningful flow estimates, rather than forcing the final \(1/4\) update block to compensate for weak coarse predictions.

% Overall, the final quantization-oriented TinyFlow model differs from the original model in four main ways: batch-normalized quantization-friendly backbone blocks, bounded residual outputs, hardware-friendly feature projection instead of dynamic L2 normalization, and bounded flow regression heads with stronger intermediate supervision. 

Overall, the final quantization-oriented TinyFlow model (we call it \textbf{QINT8\_all}) differs from the original model  (\textbf{INT8}) in four main ways:
\begin{itemize}
    \item adding batch normalization after convolutioin,
    \item changing ReLU to ReLU6,
    \item hardware-friendly feature projection instead of dynamic L2 normalization
    \item bounded flow heads and delta flows.
\end{itemize}
These changes substantially improved final quantization quality of the model.

% In our Hailo optimization experiments, the final $1/4$-resolution flow output improved from very low SNR (\textcolor{red}{needs number}) in the original model to approximately $19.6$--$20.3$ dB after the redesign.



